Right Decisions from Wrong Predictions: A Mechanism Design Alternative to Individual Calibration

Decision makers often need to rely on imperfect probabilistic forecasts. While average performance metrics are typically available, it is difficult to assess the quality of individual forecasts and the corresponding utilities. To convey confidence about individual predictions to decision-makers, we propose a compensation mechanism ensuring that the forecasted utility matches the actually accrued utility. While a naive scheme to compensate decision-makers for prediction errors can be exploited and might not be sustainable in the long run, we propose a mechanism based on fair bets and online learning that provably cannot be exploited. We demonstrate an application showing how passengers could confidently optimize individual travel plans based on flight delay probabilities estimated by an airline.

==> discussion.tex <==
\section{Discussion}

\sj{Haven't written this section very carefully, to cut if we don't have space}

\paragraph{Honesty} In a typical application where the forecaster and decision makers are separate entities, the forecaster may be incentivized to intentionally forecast the wrong probability (even if it knew the true probability $\mu_t^*$). For example, an airline could be incentivized to predict a lower probability of delay to attract passengers. The betting mechanism can potentially disincentivize the airline to predict a lower probability --- if the airline predicts a lower probability, it will lose bets on average because . On other other hand, the airline could be incentivized to predict a higher probability (to take advantage of the insurance). How to further modify the mechanism to incentivize honesty is an important open question. 

%For example, for a type of illness there are $K$ drug companies that each developed a treatment plan. Given the features of a patient (e.g. genomics sequencing data) each drug company can predict whether its drug is effective. Each patient can only undergo one treatment at a time, and must decide between the different treatment options. How can the patient trust that the drug company is making the best effort to predict the true probability? For example, the drug company could have an incentive to over-claim the effectiveness of the treatment to increase sales. Current solution is by tight regulations on what the drug company can claim about their product. 

% However, if the drug company is required to take bets based on its probability forecast, it will be incentivized to forecast the true probability. Suppose the drug company A knows that the true probability of effectiveness for a patient is $\mu_A^*$ but advertises a high probability $\mu_A > \mu_A^*$, then the drug company will on average lose bets. Conversely, if the drug company advertises $\mu_A < \mu_A^*$ it will make a profit, but then it an another company $B$ advertises $\mu_B$ and $\mu_A < \mu_B$, the patient will choose company $B$ instead. 

% In the second experiment, we do a realistic real world application of our method. There are often multiple treatments to the same illness and it is unclear which treatment will be effective. Different hospitals / drug companies can offer different treatments, and they each advertise some probability of effectiveness. How should a patient select between the different treatments?

% Suppose We simplify the problem and only consider two types of outcomes: remission or progression.  Formally for each treatment plan the patient has some loss function $l_t^k: \Ac \times \lbrace 0, 1 \rbrace \to \mathbb{R}$, we allow the loss to be different because e.g. some treatment could be more costly, or have larger side effect then others. The patients needs to select $k$ actions $a_t^1, \cdots, a_t^K \in \lbrace 0, 1\rbrace$ where only one of the $a_t^k = 1$ while others equals $0$.

% To assist the patient in making the decision, each drug company forecasts the probability of remission $\mu_t^k, c_t^k$. Suppose these probabilities are correct, then the patient lose at most $\Eb_{Y \sim \mu_t^k - c_t^k}[l(1, Y)]$ for treatment $k$, so it selects the treatment option that minimizes this value. In Figure we plot the histogram of the true utility of the patient if they adopt this strategy. 

% However, the patient may not trust the probabilities because e.g. it is only average calibrated, or drug companies have the motivation to over-claim their effect. However, if the drug company is willing to bet, then the patient knows that it lose at most $\Eb_{Y \sim \mu_t^k - c_t^k}[l(1, Y)]$. The patient can choose the company that maximizes this lower bound. 

\paragraph{Fairness} The guarantee of our mechanism has some connection with fairness, but does not equate existing notions of fairness. For example, a drug company can predict a larger interval (i.e. bigger $c_t$) for a group of patients, and that group will have worse guaranteed utility. However one benefit is that there is no hidden unfairness --- the guaranteed utility for every group is known in advance before each agent makes the decision. This is arguably better than hidden unfairness. For example, a drug company could predict favorable treatment outcome for a group of patients, but their actual treatment outcome is poor. It is another open question to study the interplay between our framework and existing notions of fairness, such as \cite{dwork2012fairness,kleinberg2016inherent,pleiss2017fairness}.


% \paragraph{Regret} A different type of guarantee is low regret 
% \begin{align*}
%     \Eb[L(\phi_B(\mu(X), c(X); X); X)] - \Eb\left[ \inf_{a \in \Ac} L(a, X) \right]  \numberthis\label{eq:regret_definition}
% \end{align*}
% However, vanishing regret is impossible to guarantee in general. We can construct two distributions --- $Y \mid x$ is deterministic, and $Y \mid x$ is stochastic --- such that there is no way to distinguish between these two distributions based on a finite dataset. The optimal action $\arg\inf_{a \in \Ac} L(a, X) $ can be different for the two distributions, which implies that we cannot guarantee selection of the optimal action based on the finite dataset. 


% Even though we do not guarantee the regret, we empirically verify that agents select near-optimal actions. Note that evaluation of regret is only possible if the true conditional probability is known. Only the MNIST dataset satisfy this requirement because the labels are synthetically generated from a known distribution. % which we can compute only for the MNIST dataset. 


\paragraph{Interpretation of Individual Probability} In Protocol 2 we consider the interaction between a single forecaster and multiple decision makers, and derive the guarantee in Proposition~\ref{prop:decision_guarantee} for decision makers. This could be generalized as: if there is an agent who is willing to back a probability forecast $\mu_t, c_t$ by accepting bets, then another agent can use this probability forecast \textit{as if it were the correct probability}. 

% This could also be understood figuratively. The meaning of an individual probability is that  
% Discuss that the forecaster-decision maker division can be interpreted either literally or figuratively. 

% \subsection{Case Study: Online Advertising} 

% A ad provider can show ads on its website for a fee of $c'_t$ and is trying to convince advertisers to buy the ad slots. An advertiser wants to know the probability the ad has the desired effect (e.g. an customer clicks into the link to buy a product). For example, let $y$ denote the variable that indicates the desired effect, and $a$ is the indicator of whether the advertiser purchases the ad slot. The loss of the advertiser would be $l(y=1, a=1) = -r_t + c'_t$ and $l(y=0, a=1) = c'_t$ which is just the cost of the ad. 

% Suppose the provider is providing service to many advertisers, it will have lots of data to predict the desired outcome . Based on the data it predicts $\mu_t, c_t$. The advertiser can offer a contract: the advertiser can choose some $g_t > 0$, if $y_t > \mu_t$ (e.g. website browser clicks into the ad and buys the product) then the provider charges an additional $g_t (1 - \mu_t + c_t)$, otherwise if $y_t < \mu_t$ the provider charges additional $ g_t (c_t - \mu_t)$.

% Under this contract if the advertiser chooses to use $g_t = -r_t$, then
% %then if $y_t = 1$ then the advertiser receives utility $r_t$ from the ad click, and pays $c_t' + r_t(1 - \mu_t + c_t)$; if $y_t = 0$ then the advertiser has no utility from ad click, and pays $c_t' + r_t(c_t - \mu_t)$
% % \begin{align*}
% %     -r_t + c_t' + r_t (1 - \mu_t + c_t) 
% % \end{align*}
% % if $y = 0$ 
% the guaranteed loss would be 
% $
%     - (\mu_t - c_t) r_t + c'_t  
% $
% In other words, the provider can guarantee that the utility of the advertiser as if the click probability is correct. The advertiser should use the provider if the guaranteed loss is negative, or $c_t' \leq (\mu_t - c_t)r_t$.


% Alternatively if the advertiser chooses to use $g_t = \frac{c'_t}{\mu_t - c_t}$ then this is equivalent to the forecast not paying if the ad has no effect, and pay $c_t' + \frac{1 - \mu_t + c_t}{\mu_t - c_t}$ if the ad is effective. 

% In either case, the provider always makes a profit of $\sum_{t=1}^T c'_t + o(T)$. However for different choice of $g_t$ the advertiser can get different types of guarantees. 



% \sj{To do into the appendix}

% TO model the ground truth function $x_t \to \mu_t^{k*}$ we use a random neural network and normalize its output to be marginally a uniform distribution. We also assume a random treatment price $p^k$ for each treatment that's uniformly drawn from an. The patient loss function when the treatment is ineffective $l_0: x_t, k \to \mathbb{R}$ we also use a random neural network, and the loss function when the treatment is effective $l_1 = l_0 + \delta l$ where $\delta l$ is another random neural network that has positive outputs. 

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> newer_old.tex <==

\glinear*

\begin{proof}[Proof of Theorem~\ref{thm:g_linear_only}, Part I]
We explicit construct such a family of $\Fc$. We require $f$ to be differentiable in $\theta$. Suppose $\theta^* = \arg\inf_\theta \Eb[(f_\theta(X) - Y)^2]$ we have by the first order condition of optimality, $\forall i=1, \cdots, m$
\begin{align*}
    \Eb\left[ \frac{\partial}{\partial \theta_i} f_{\theta^*}(X) (f_{\theta^*}(X) - Y) \right] = 0
\end{align*}
Given some choice of $\Gc \subset \lbrace \sum_i \phi_i h_i, \phi_i \in \mathbb{R} \rbrace$ we want to choose $f$ such that there exists some invertible $A \in \mathbb{R}^{m \times m}$ and $\forall x \in \Xc$
\begin{align*}
     \frac{\partial}{\partial \theta_i} f_{\theta^*}(x)  = \sum_j A_{ij} h_j (x, f_{\theta^*}(x))
\end{align*}
but since $\theta^*$ is determined by the underlying distribution and cannot be controlled we want to choose $f$ such that $\forall x \in \Xc, \theta \in \mathbb{R}^m$ 
\begin{align*}
     \nabla_\theta f_{\theta}(x)  = A(\theta) h (x, f_{\theta}(x))
\end{align*}
Note that this is a partial differential equation, where a solution is a pair of functions $f, A$ that satisfies the differential equation. 

We consider the following PDE
\begin{align*}
    \nabla_\theta \psi(\theta)  = A(\theta) h(\psi(\theta))
\end{align*}
% Choose any flow line $\gamma_{\theta}: \mathbb{R} \to \Theta$ where $\gamma_{\theta}(0) = \theta$ and $\gamma_\theta'(t) = \phi(t)$. Obverse that for any choice of $\theta_0, \theta_1$ we have $\gamma_{\theta_1}(t) - \gamma_{\theta_0}(t) = \theta_1 - \theta_0$. Choose some direction $v \in \Theta$, and let $v^\perp(\theta_0)$ denote the linear subspace $v^T(\theta - \theta_0) = 0$ and define the collection of all $\gamma_{\theta}, \theta \in v^\perp(\theta_0)$. We can choose $\psi(\theta) = \gamma^{-1}(\theta)$. 
Choose any unit $L_2$ length vector $v$ in $\Theta$ we define the new variable $\lambda = v^T \theta$ and consider the one-dimensional ODE 
\begin{align*}
    \tilde{\psi}'(\lambda) = v^T \phi(\tilde{\psi}(\lambda))
\end{align*}
which is separable, and we can solve it by 
\begin{align*}
    \lambda = \int_{0}^{\tilde{\psi}(\lambda)} \frac{1}{v^T \phi(y)} dy
\end{align*}
We can extend this $\psi$ to a solution the original PDE. Consider 
\begin{align*}
    \psi(\theta) = \tilde{\psi}(v^T \theta)
\end{align*}
it is easy to check that this solution satisfies the PDE because
\begin{align*}
    \nabla_\theta \psi(\theta) = \tilde{\psi}'(v^T \theta) v = v^T \phi(\psi(\theta)) v = vv^T \phi()
\end{align*}
% \begin{lemma}
% If the functions $\phi_i: \mathbb{R} \to \mathbb{R}$ satisfies global Lipshitzness $|\phi(x) - \phi(x')| \leq C|x - x'|$ and linear growth $\phi(x) \leq C(1 + |x|)$ then the differential equation 
% \begin{align*}
%     \frac{\partial}{\partial \theta_i} \psi(\theta)  = \phi_i (\psi(\theta))
% \end{align*}
% has a continuous solution.
% \end{lemma}

% We construct a sequence of solutions $\psi^1, \psi^2, \cdots$ where 
% \[ \psi^{k+1} = \int \phi_i(\psi^k(\theta)) \]


\end{proof} 
\begin{proof}[Proof of Theorem~\ref{thm:g_linear_only}, Part II]
We first show that there exists $g_1, \cdots, g_{m+1} \in \Gc$ that are linearly independent. Suppose we cannot do this, then it must be that as soon as we choose $h_1, \cdots, h_m \in \Gc$ all other $g \in \Gc$ are linear functions of $h_1, \cdots, h_m$, but this would imply $\Gc \subset \lbrace \sum_i \phi_i h_i, \phi_i \in \mathbb{R} \rbrace$, which is a contradiction to the condition. 

Since $g_1, \cdots, g_{m+1}$ are linearly independent, consider the "matrix" $G_{jx} = g_j(x)$ which must be a matrix of rank $m+1$. Because this matrix has $m+1$ linearly independent rows, it must also have $m+1$ linearly independent columns. Therefore, it must have an $(m+1) \times (m+1)$ sub-matrix with rank $m+1$. In other words, there must be some $x_1, \cdots, x_{m+1} \in \Xc$ such that the matrix
\begin{align*}
    \tilde{G} = \left( \begin{array}{llll} g_1(x_1) & g_1(x_2) &\cdots & g_1(x_{m+1}) \\
    &&\cdots &\\
    g_{m+1}(x_1) & g_{m+1}(x_2) & \cdots & g_{m+1}(x_{m+1}) \end{array} \right)
\end{align*}
is full rank. 

Choose $X$ as the uniform distribution on $\lbrace x_1, \cdots, x_{m+1} \rbrace$ and use the new notation 
\begin{align*}
    \tilde{f}_\theta &= (f_\theta(x_1), \cdots, f_\theta(x_{m+1}))^T \\
    \tilde{\mu} &= (\Eb[Y \mid x_1], \cdots, \Eb[Y \mid x_{m+1}])
\end{align*} 
then we can rewrite the following expression in matrix notation as
\begin{align*}
    \left( \begin{array}{l} \Eb[g_1(X) (f_\theta(X) - Y)] \\ \cdots \\ \Eb[g_{m+1}(X) (f_\theta(X) - Y)]  \end{array} \right) = \frac{1}{m+1} (\tilde{G} \tilde{f}_\theta - \tilde{G} \tilde{\mu})
\end{align*}
Suppose we always have $\inf_{f \in \Fc} \sup_{g \in \Gc} \Eb[g(X) (f_{\theta}^*(X) - Y)] > 0$, this would imply for some $\theta^*$
\[ \forall j =1, \cdots, m+1 \qquad \Eb[g_j(X) (f_\theta(X) - Y)] = 0 \]
which implies $\tilde{G} \tilde{f}_\theta = \tilde{G} \tilde{\mu}$ which because $\tilde{G}$ is full rank is equivalent to $\tilde{f}_{\theta^*} = \tilde{\mu}$. However, this is impossible for every choice of $\tilde{\mu}$ because the map $\theta \mapsto \tilde{f}_{\theta^*}$ is a map $\mathbb{R}^m \to [0, 1]^{m+1}$ while $\tilde{\mu}$ can be any vector in $[0, 1]^{m+1}$. $[0,1]^{m+1}$ and $\mathbb{R}^m$ are not homeomorphic, hence a contradiction. 
\end{proof}

\begin{proof}[Proof of Corollary~\ref{cor:optim_equivalence}]
Suppose there exists some $g \in \Gc$ such that for some $f_\theta \in \Fc$, i.e. there exists $c > 0$ such that
\begin{align*}
    \Eb[g(X) (f_\theta(X) - Y)] = c > 0
\end{align*}
then we can construct a $\tilde{f} = f_\theta - \delta g \in \Fc$ and have 
\begin{align*}
    \Eb[(\tilde{f}(X) - Y)^2 - (f_\theta(X) - Y)^2] &= \Eb[-2 \delta g(X)(f_\theta(X) - Y) + \delta^2 g(X)^2] \\
    &= -2\delta c + \delta^2 \Eb[g(X)^2]
\end{align*}
When $\delta$ is small enough we have $\Eb[(\tilde{f}(X) - Y)^2 - (f_\theta(X) - Y)^2] < 0$, so it is impossible to have 
\begin{align*}
    f_\theta = \arg\min_{f \in \Fc} \Eb[(f(X) - Y)^2] 
\end{align*}
\end{proof}


\begin{proof}[Proof of Proposition~\ref{prop:lower_bound}]
Suppose we have two sets of samples $x_1, \cdots, x_t, \cdots, x_T$ and $x_1, \cdots, x_t', \cdots, x_T$ that only differ in one sample $x_t$. Let $\hl(g, f, c)$ be Eq.(\ref{eq:empirical_error}) computed on the first set of samples and $\hl'(f, c)$ be Eq.(\ref{eq:empirical_error}) computed on the second set of samples. Then we have by Jensen inequality
\begin{align*}
    |\hl(f, c) - \hl'(f, c)| &\leq \sup_{g \in \Gc} \left\lvert \frac{1}{T} g(x_t) (f(x_t) - y_t) - |g(x_t)| c(x_t) - g(x_t') (f(x_t') - y_t') + |g(x_t')| c(x_t') \right\rvert \\
    &\leq 2M/T
\end{align*}
By Mcdiarmid inequality we have
\begin{align*}
    \Pr\left[ \hl(f, c) \leq \Eb[\hl(f, c)]  - s \right] \leq e^{-Ts^2/2M^2} 
\end{align*}
But since $\Eb[\hat{l}(f, c)] \geq l(f, c)$ we have 
\begin{align*}
    \Pr\left[ \hl(f, c) \leq l(f, c)  - s \right] \leq e^{-Ts^2/2M^2} 
\end{align*}
We can rearrange to finish the proof of Lemma 2. 
\end{proof}




\subsubsection{Learning Calibrated Forecasters}

We can directly optimize $f$ by minimizing Eq.(\ref{eq:calibration_error}) 
\begin{align*}
    \inf_f \sup_{g \in \Gc} \Eb[g(X, \mu(X))(\mu(X) - \Eb[Y \mid X]) - |g(X, \mu(X))|c(X)]  
\end{align*}
However, this is a minimax optimization and can suffer from stability problems in practice. Instead of minimax optimization, we show that it is usually sufficient to minimize $L_2$ error for the right parametric family $f_\theta$. 




% The hope is that whether we can do better to optimize directly $g(x) (f(x) - y)$, and the following proposition provides strong argument against this. 

% \begin{prop} 
% Suppose $f_\theta$ is continuous in $\theta \in \mathbb{R}^N$, and $g_\phi$ is continuous in $\phi \in \mathbb{R}^M$ and $\lbrace \frac{\partial}{\partial \phi_1} g_\phi(X), \cdots \frac{\partial}{\partial \phi_M} g_\phi(X) \rbrace$ are not linearly independent functions. $\min_\theta \max_\phi \Eb[ g_\phi(X) (f_\theta(X) - Y) ] > 0$ in general if $N < M$. 
% \end{prop} 
% \begin{proof}
% To avoid technical difficulty we consider $\Xc$ that contain a finite number of elements. 
% Consider the minimax game $\min_\theta \max_\phi \Eb[ g_\phi(X) (f_\theta(X) - Y) ]$. Suppose $\theta \in \mathbb{R}^d$ but $\phi \in \mathbb{R}^{d+1}$. If there exists some $\theta^*$ we have $\forall \phi, \Eb[ g_\phi(X) (f_\theta(X) - Y) ] = 0$  then we must have
% \begin{align*}
%     \frac{\partial}{\partial \phi_i}  \Eb[ g_\phi(X) (f_\theta(X) - Y) ]  , i=1, \cdots, d+1
% \end{align*}
% This can be equivalently written as 
% \begin{align*}
%     \Eb\left[ \frac{\partial}{\partial \phi_i}  g_\phi(X) f_\theta(X) \right] = \Eb\left[ \frac{\partial}{\partial \phi_i}  g_\phi(X) \Eb[Y \mid X] \right] 
% \end{align*}
% The range of $\frac{\partial}{\partial \phi_i}  g_\phi(X) f_\theta(X)$ in the space $\Xc \to \mathbb{R}$ is a $d$-dimensional manifold. On the other hand, the range (as we vary $\Eb[Y \mid X]$ of $ \frac{\partial}{\partial \phi_i}  g_\phi(X) \Eb[Y \mid X]$ is a $ \left\lVert \frac{\partial}{\partial \phi_i}  g_\phi(X) \right\rVert_0$-dimensional manifold (where $\lVert \cdot \rVert_0$ denote the number of non-zero elements). A continuous $d$-dimensional manifold cannot cover a manifold of higher dimension. 
% \end{proof}
% In addition, we know that if some $\theta^*$ is selected, and if $\Gc$ contains all the gradients $\frac{\partial}{\partial \theta_j} f_{\theta^*}(x)$ then we cannot have calibration unless $\theta^*$ is the $L_2$ minimizer. 

% Observe that this optimization problem has linear objective (in $\nu$) and linear constraints. In particular, there are $K+1$ variables and $K$ constraints. Therefore the set of 




% \begin{prop}
% \label{prop:g_linear_only}
% Choose some $\Xc$, $\Fc = \lbrace f(\cdot, \theta): \Xc \to \mathbb{R}, \theta \in \mathbb{R}^m \rbrace$ where $f$ is continuous in $\theta$ and $\Gc$ be a set of functions such that whenever $g \in \Gc$, $-g \in \Gc$ we have
% \begin{enumerate}
%     \item If $f$ is differentiable in $\theta$, then for every distribution, there exists some $h_1, \cdots, h_m: \Xc \to \mathbb{R}$ such that if $\Gc \subset \lbrace \sum_i \phi_i h_i, \phi_i \in \mathbb{R} \rbrace$ then $\inf_{f \in \Fc} \sup_{g \in \Gc} \Eb[g(X) (f_\theta(X) - Y)] = 0$
%     \item If there do not exist $h_1, \cdots, h_m: \Xc \to \mathbb{R}$ such that $\Gc \subset \lbrace \sum_i \phi_i h_i, \phi_i \in \mathbb{R} \rbrace $ then there exists a distribution such that $\inf_{f \in \Fc} \sup_{g \in \Gc} \Eb[g(X) (f_\theta(X) - Y)] > 0$
% \end{enumerate}
% \end{prop}

\begin{definition}
For some set $\Gc \subset \lbrace \Xc \times [0, 1] \to \mathbb{R} \rbrace$ we say $\Gc$ has rank $m$ if for the smallest $m \in \mathbb{N}$ there exists $h_1, \cdots, h_m: \Xc \times [0, 1] \to \mathbb{R}$ such that $\Gc \subset \lbrace \sum_i \phi_i h_i, \phi_i \in \mathbb{R} \rbrace$. If no such $m$ exist we say $\Gc$ has rank $\infty$. 
\end{definition}
\begin{restatable}{theorem}{glinear}
\label{thm:g_linear_only}
Choose any set $\Gc \subset \lbrace \Xc \times [0, 1] \to \mathbb{R} \rbrace$ then 
\begin{enumerate}
    \item If $\mathrm{rank}(\Gc) \leq m$ then there exists some $\Fc = \lbrace f_\theta: \Xc \to \mathbb{R}, \theta \in \mathbb{R}^m \rbrace$ such that choose $\theta^* = \arg\inf_\theta \Eb[(f_\theta(X) - Y)^2]$ we have $\sup_{g \in \Gc} \Eb[g(X, f_\theta(X))(f_\theta(X) - Y)] = 0$. 
    \item If $\mathrm{rank}(\Gc) > m$ then for any $\Fc = \lbrace f_\theta: \Xc \to \mathbb{R}, \theta \in \mathbb{R}^m \rbrace$ where $f_\theta$ is continuous in $\theta$, there exists a distribution such that $\inf_{f \in \Fc} \sup_{g \in \Gc} \Eb[g(X, f_\theta(X)) (f_\theta(X) - Y)] > 0$
\end{enumerate}
\end{restatable}

For part I of the theorem we use an existence proof where $f_\theta$ is the (guaranteed-to-exist) solution of a PDE. For several simple $\Gc$ we explicitly construct $\Fc$ which has a closed form solution and can be directly used as the forecast model. We leave as an open question how to do this in general. 




% \begin{corollary} Let $\Fc = \lbrace f(\cdot; \theta): \Xc \to \mathbb{R} \rbrace$ be a family of differentiable functions indexed by $\theta \in \mathbb{R}^K$. Let
% $
%     \theta^* = \arg\min_{\theta} \Eb[(f_\theta(X) - Y)^2]
% $ and $f_{\theta^*}(X) \in (0, 1)$, we have
% \begin{enumerate}
% \item If $g(X) = \phi^T \nabla_\theta f_{\theta^*}(X)$ for some $\phi \in \mathbb{R}^K$ then $\Eb[g(X) (f_{\theta^*}(X) - Y)] = 0$  
% \item If $g(X) \neq \phi^T \nabla_\theta f_{\theta^*}(X)$ for all $\phi \in \mathbb{R}^K$ then there exists a distribution such that $\Eb[g(X) (f_{\theta^*}(X) - Y)] > 0$  
% \end{enumerate}
% \end{corollary}
% \begin{proof}
% If: This is easy to see because by the first order necessary condition for optimality we have 
% \begin{align*} 
% \Eb[g(X) (f_{\theta^*}(X) - Y)] =  \phi^T \Eb[\nabla_\theta f_{\theta^*}(X) \left( f_{\theta^*}(X) - Y\right) ] = \phi^T \Eb[\nabla_\theta \left(f_{\theta^*}(X) - Y\right)^2 ] = 0
% \end{align*}

%Only if: this is a simple corollary of Proposition~\ref{prop:g_linear_only}. 
% Only if: Choose $p(X)$ to be uniformly supported on only $K+1$ points $\lbrace x_0, \cdots, x_K \rbrace$, and denote $\nu_i = \Eb[Y \mid X=x_i]$. Choose any $g$ such that $g(X) \neq \phi^T \nabla_\theta f_{\theta^*}(X)$ for all $\phi \in \mathbb{R}^K$, and denote $\mu_i = f_{\theta^*}(x_i)$. We would like to construct some $\nu$ such that 
% \begin{align*}
%     \theta^* = \arg\inf_{\theta} \sum_i \Eb_{Y \sim \nu_i}[(f_\theta(x_i) - Y)^2]
% \end{align*}
% taking the first order optimality condition 
% Define the optimization problem
% \begin{align*}
%     \max_{\nu \in [0, 1]^{K+1}} \qquad &\sum_i g(x_i) (f_{\theta^*}(x_i) - \nu_i) \\
%     s.t. \qquad &\sum_i \frac{\partial}{\partial \theta_j}f_{\theta^*}(x_i) (f_{\theta^*}(x_i) - \nu_i) = 0, \forall j=1, \cdots, K 
% \end{align*}
% Let $s(x)$ be the projection of $g(x)$ onto the orthogonal complement of the subspace spanned by $\lbrace \frac{\partial}{\partial \theta_i}f_{\theta^*}(x_i) \rbrace$. Then choose $\nu_i = f_{\theta^*}(x_i) - \epsilon s(x_i)$. It is easy to see that for sufficiently small $\epsilon$, $\nu_i \in [0, 1]$ and it is a witness that shows that the value of the optimization problem is positive. 
%\end{proof}


% \begin{corollary} \label{cor:optim_equivalence}
% For uniformly bounded set of functions $\Gc \subset \lbrace \Xc \to \mathbb{R} \rbrace$, a function $f^*: \Xc \to [0, 1]$ is calibrated with respect to $\Gc$ if there exists $\Fc \subset \lbrace \Xc \to \mathbb{R} \rbrace$ such that
% \begin{enumerate}
%     \item $\forall f \in \Fc, g \in \Gc$, $f + g \in \Fc$
%     \item $f^* = \arg\min_{f \in \Fc} \Eb[(f(X) - Y)^2]$
% \end{enumerate} 
% \end{corollary}
% In words, $f$ is calibrated if it is the quadratic loss minimizer among a sufficiently large set of functions. TODO: the L2 might be generalized to other Bregman divergences. TODO: there is a stronger version where 1 only needs to hold in a local Taylor expansion.

% \paragraph{Example: All functions} When $\Gc$ is the set of all functions, choosing $\Fc$ as the set of all functions also satisfies the condition of Theorem~\ref{thm:g_linear_only}.

\paragraph{Example: Standard Calibration} Suppose $\Gc$ is the set of all functions that only depend on $\mathrm{Dist}^m(f_\theta(x))$ where $\mathrm{Dist}^m$ is any function $[0, 1]$ to $[m]$ (interpreted as a discretization map). Then the corresponding set of $\Fc$ is $f_\theta(x) = s_\phi(\mathrm{Dist}^m(\tilde{f}(x)))$ where $s_\phi$ is the set of all functions $[m] \to [0, 1]$ where $s_\phi(i) = \phi_i$. This corresponds to the histogram binning (re)calibration algorithm. 

\paragraph{Examples: Linear Regression} %When $\Gc$ is the set of linear functions of $x$, choosing $\Fc$ as the set of linear functions satisfies the conditions of Theorem~\ref{thm:g_linear_only}. %On the other hand, if we choose $\Fc$ as the set of linear-Sigmoid functions, the condition of Proposition~\ref{prop:optim_equivalence} is not satisfied (even though this is a more natural choice since $Y \in [0, 1]$). (Note: empirically verified)
When $\Gc$ is a linear function on some feature space $\Gc = \lbrace \phi_i h_i(x) \rbrace$ then choosing $\Fc$ as the set of linear functions on the same features satisfies the conditions of Theorem~\ref{thm:g_linear_only}
% \paragraph{Example: General feature space linear regression} Choose any feature function $s: \Xc \to \mathbb{R}^M$ and it if we choose $\Gc = \lbrace g_\phi: x \mapsto \langle s(x), \phi \rangle, \phi \in \mathbb{R}^M \rbrace$ then we can always construct some family of $\Fc$ such that minimizing $L_2$ error is sufficient to guarantee calibration relative to $\Gc$. In particular as long as $\Fc$ contains $\Gc$ then the condition is satisfied. On the other hand, if $\Gc$ contains functions $g_\phi$ that is not linear (or piece-wise linear) in $\phi$, then as Proposition~\ref{prop:g_linear_only} shows, it is in general impossible to find some set of functions $\Fc$ that can satisfy calibration. 

\paragraph{Counter Example} Choose $\Gc = \lbrace e^{\langle \phi, x \rangle}, \phi \in \mathbb{R}^d \rbrace$ then the linear rank of $\Gc$ is infinite. 

% \subsection{Learning Sound Forecasters}

% \begin{align*}
%     \max_g \qquad &\Eb[g(X)(f(X) - \Eb[Y \mid X]) - |g(X)| c(X) ] \\
%     \min_c \qquad &\Eb[c(X)] \\
%     s.t.\qquad  & \Eb[g(X)(f(X) - \Eb[Y \mid X]) - |g(X)|c(X)] \leq 0 \numberthis\label{eq:calibration_constraint}
% \end{align*}




\subsection{PAC Bound}
Nevertheless to compare with previous approaches, we can still bound the number of samples necessary to prove that a forecaster is sound. 
Define the Radamacher complexity of $\Gc$ by 
\begin{align*}
    \Rc_T(\Gc) := \Eb_{b_t \sim \mathrm{Ber}} \left[ \sup_{g \in \Gc} \frac{1}{T} \sum_t b_t g(x_t) \right]
\end{align*}
then we have the following theorem
\begin{prop} 
\label{prop:radamacher}
With $1-\delta$ probability (over random instantiations of the dataset)
\begin{align*}
    \Pr\left[ \hat{l}(f, c) \geq l(f, c) + 2\Rc_T(\Gc) + \sqrt{\frac{2M^2}{T} \log \frac{1}{\delta}}  \right] \leq \delta
\end{align*}
\end{prop}

\subsection{Relationship to Histogram Binning}
If $g$ is a function of the discretized values then we get the histogram binning approximation for standard calibration. More formally, 
suppose we discretize the values of $\mu \in [0, 1]$ into $0 = c_1 < \cdots < c_B = 1$ and choose $\Gc: [B] \to \mathbb{R}$, denote $c_t$ as the random variable where $c_t = i$ if $c_i \leq c_t < c_{i+1}$, then 
\begin{align*}
    \Rc(\Gc) &= \Eb[\sup_{g \in \Gc} \frac{1}{T} \sum_t b_t g(\mu_t)] = \frac{1}{T} \Eb\left[ \sum_i \left\lvert \sum_{t, c_t = i} b_t \right\rvert \right] = \frac{1}{T} \sum_i \Pr[c_t = i] \sqrt{T \Pr[c_t = i]} \\
    &= \frac{1}{\sqrt{T}} \sum_i \Pr[c_t = i] \sqrt{\Pr[c_t = i]}
\end{align*}
The term $\sum_i \Pr[c_t = i] \sqrt{\Pr[c_t = i]}$ is similar to entropy. Suppose there is an $i$ where $\Pr[c_t = i] = 1$ then the term takes its minimum value of 1. Conversely if $\Pr[c_t = i] = 1/B$ for all $i$ then the term takes its maximum value of $\sqrt{B}$. By combining with Proposition~\ref{prop:radamacher} we obtain a sharper sample complexity bound than standard analysis of histogram binning (Maybe?). 


\subsubsection{Uniform Convergence}

Define the notation 
\begin{align*} l(f, c) =  \sup_{g \in \Gc} \Eb[g(X)(f(X) - \Eb[Y \mid X]) - |g(X)|c(X)] \numberthis\label{eq:calibration_error} \end{align*}
This can be thought of as a measurement of the "calibration error".

Suppose we are given $T$ i.i.d. data $x_t, y_t \sim p^*$, can we use them to verify that a forecaster $f$ is sound with respect to $\Gc$. We can compute 
\begin{align*}
    \hat{l}(f, c) := \sup_{g \in \Gc} \frac{1}{T} \sum_{t=1}^T g(x_t) (f(x_t) - y_t) - |g(x_t)| c(x_t) \numberthis\label{eq:empirical_error}
\end{align*} 
Note that $\Eb[\hat{l}(f, c)] \geq l(f, c)$, so if empirically a forecaster is sound ($\hat{l}(f, c) \leq 0$) then w.h.p. it is sound in expectation. This is formalized in a simple Lemma which can be easily proved by showing bounded difference and applying Mcdiarmid inequality. 
\begin{prop} 
\label{prop:lower_bound}
With $1-\delta$ probability (over random instantiations of the dataset)
\begin{align*}
    \Pr \left[\hl(f, c) \leq l(f, c) - \sqrt{\frac{2M^2}{T} \log \frac{1}{\delta}} \right] \leq \delta
\end{align*}
\end{prop}

A big benefit of this proposition is that there is no need to explicitly bound uniform convergence in practice. As long as the skeptic can be optimized to global solutions, we are automatically guaranteed that soundness is at least as good as $\hat{l}(g, f, c)$. 


==> old.tex <==
We have an expectation matching theorem that is an extension of Ali's paper. 
\begin{prop}
\label{prop:expectation_matching}
Suppose a forecaster $\mu, c$ is sound with respect to $\Gc$ then for any function $\psi: \Xc \times \Yc \to \mathbb{R}$ such that $\psi(\cdot, 1) - \psi(\cdot, 0) \in \Gc$  
\begin{align*}
    \left\lvert \Eb_{X \sim p^*, Y \sim \mu(X)}[\psi(X, Y)] - \Eb_{X, Y \sim p^*}[\psi(X, Y)] \right\rvert \leq  \Eb_{X \sim p^*}[|\psi(X, 1) - \psi(X, 0)| c(X)]
\end{align*}
\end{prop}

To recover the special case in Ali's paper we can simply observe that $\psi$ does not depend on $x$ so it is automatically true that $\psi(\cdot, 1) - \psi(\cdot, 0) \in \Gc$ when $\Gc$ is the corresponding set for standard calibration. 




% \paragraph{Statistical assumptions} To provide guarantees in the offline setup we need to assume standard statistical machine learning assumptions i.e. there exists some true distribution $X, Y \sim p^*$ and all the data (both the offline training data and test data) are drawn i.i.d. according to this distribution. 


We say that a function class $\Fc$ is calibrated with respect to loss function $l$ and decision rule $\phi$ if $\Fc$ is calibrated with respect to $\Gc$ and 
\begin{align*}
    x \mapsto l(\phi(\mu(x), c(x), x), x, 1) - l(\phi(\mu(x), c(x), x), x, 0) \in \Gc
\end{align*} 

\paragraph{g is linear}:
Suppose $g: x \mapsto w^T x$, then to satisfy 
\[ \Eb[w^T X (f(X) - \Eb[Y \mid X]) - |w^T X| c(X)] \leq 0 \]
it suffices to have
\begin{align*}
    w^T \Eb[ X (f(X) - \Eb[Y \mid X]) ] &\leq \Eb[|w^T X| c(X)]  \\
    &= \Eb[w^T X c(X) \mid w^T X \geq 0] \Pr[w^T X \geq 0] -  \Eb[w^T X c(X) \mid w^T X < 0] \Pr[w^T X < 0] 
\end{align*} 
We can move the $w$ out of the expectation and conclude that the above is equivalent to 
\begin{align*}
    \Eb[ X (f(X) - \Eb[Y \mid X]) ] \leq \Eb[X c(X) \mid w^T X \geq 0] \Pr[w^T X \geq 0] -  \Eb[ X c(X) \mid w^T X < 0] \Pr[w^T X < 0] 
\end{align*}
or equivalently 
\begin{align*}
    \Eb[ X f(X)]  - \Eb[XY]  \leq \Eb[X c(X) \mid w^T X \geq 0] \Pr[w^T X \geq 0] -  \Eb[ X c(X) \mid w^T X < 0] \Pr[w^T X < 0] 
\end{align*}

Other thoughts: $g_t$ could be functions from the decision loss ($l_t$ in next section). 


There is a simple generalization to multiclass classification

\begin{enumerate}
    \item Nature reveals $x_t$ and chooses a distribution $p^*_z$ on $[N]$ without revealing it. 
    \item Classifier predicts $z_t \in [N]$
    \item Forecaster predicts $\mu_t, c_t$
    \item Agent $t$ has loss function $l_t: [N] \times \lbrace 0, 1 \rbrace \times \Ac \to \mathbb{R}$ 
    \item Nature samples $y_t = \Pr_{z \sim p^*_z}[z_t = z]$ 
    \item Forecaster loss is $l_t(z_t, y_t, \tilde{a}^*)$
\end{enumerate}

In other words, the loss function can depend on $z_t$. The loss if the prediction $z_t$ is correct, and the loss if the prediction is incorrect. This is a somewhat restricted generalization, but it is immediate compatibility with the rest of the paper. For example, in an driving task, the classifier could be classifying the object in front, and $a$ can be decisions to accelerate or decelerate. Assuming the classification is correct, depending on whether the classification label is drivable surface / some obstacle, etc, there can be a corresponding loss for each $a$. On ther other hand, if the classification is incorrect, then the car should always decelerate. 

Option 1: defensive forecasting method. We can run the following algorithm
\begin{enumerate}
    \item Let $\Dc = \emptyset$ and $b_1 = 0$
    \item For $t = 1, \cdots, T$
    \begin{enumerate}
        \item Choose $\theta_t = \arg\min \sum_{\tau = 1}^{t-1} (f_\theta(x_\tau) - y_\tau)^2$ and set $f_t = f_{\theta_t}(x_t)$
        \item Choose $\lambda_t = \arg\min_\lambda \sum_{\tau=1}^{t-1} (g_\tau (f_{\theta_t}(x_\tau) - y_\tau) + |g_\tau|c_\tau(x_\tau)$ and set $c_t = c_{\lambda_t} + b_0$
        \item Nature/Skeptic reveal $r_t = g_t (f_t - y_t) - |g_t| c_t$
        \item If $\sum_{t=1}^T r_t > 0$ set $b_{t+1} = b_t + \epsilon / T$; otherwise set $b_{t+1} = b_t - \epsilon/T$
    \end{enumerate}
\end{enumerate}


\subsection{The Revised Protocol} 


At time $t = 1, \cdots, T$
\begin{enumerate}
    \item Nature reveals $x_t \in \Xc$ and chooses $\mu_t^* \in [0, 1]$ without revealing it
    \item Forecaster predicts $\mu_t$, insurer predicts $c_t$ 
    \item Agent $t$ has loss function $l_t: \lbrace 0, 1 \rbrace \times \Ac \to \mathbb{R}$
    \begin{enumerate}
        \item Agent Bayesian loss is 
        \[ \tilde{L}_t(a) = \mu_t l_t(1, a) - (1 - \mu_t) l_t(0, a) \]
        and agent selects $\tilde{a}^*_t = \arg\inf_{a \in \Ac} \tilde{L}(a)$
        \item Agent chooses $g_t \in \mathbb{R}$
    \end{enumerate}
    \item Nature samples $y_t \sim \mathrm{Bernoulli}(\mu_t^*)$ and reveals $y_t$
    \item Agent incurs actual loss 
    $
        l_t^* = l_t(y_t, \tilde{a}^*) - g_t(y_t - \mu_t) + |g_t| c_t 
    $
    and agent surprise is
    \begin{align*}
        \hat{s}_t = l_t^* - \tilde{L}_t(\tilde{a}^*) 
    \end{align*}
    \item Insurer loss is given by $g_t(y_t - \mu_t) - |g_t|c_t$
\end{enumerate}


However, the impossibility result only applies if the protocol is strictly followed. Here we consider a variation: there is a third player we call an insurer. At each iteration the insurer pays the agent a certain amount $i_t$ (that can be positive or negative). The new loss of the agent $\hat{L}$ is given by the $L(a)$ plus the amount it receives from the insurer, i.e. 
\[ \hat{l}_t^* = l_t^* + i_t \] 
and as before we define agent surprise as 
\begin{align*}
    \hat{s}_t = \hat{l}_t^* - \tilde{L}_t(\tilde{a}^*) \numberthis\label{eq:surprise_def_1}
\end{align*} 
Compared to Eq.(\ref{eq:surprise_def_0}) the only difference is that the agent receives an additional payment from the insurer. We would still like to guarantee that 
\begin{align*}
    \Eb[\hat{s}_t] \leq |l_t(1, a) - l_t(0, a)|c_t  \numberthis\label{eq:decision_guarantee_1}
\end{align*}
In other words, given that the agent agrees to receive payment $i_t$ from the insurer, the difference between what it expects to get and what it actually gets is still bounded. 

Note that the insurer can always pay the agent a sufficiently large positive amount such that Eq.(\ref{eq:decision_guarantee_1}) is trivially satisfied. The difficulty here is that we want to obtain Eq.(\ref{eq:decision_guarantee_1}) \textbf{for free} --- the amount the insurer gives to the agent is the insurer's loss, and we want the insurer's loss to be upper bounded by a constant (even as $t \to \infty$). 

To summarize we want to satisfy the following desiderata: 
\begin{enumerate}
    \item The insurer cannot lose more than a constant amount (as $t \to \infty$), even when nature is adversarial, or when the agent does not follow the protocol. 
    \item Eq.(\ref{eq:decision_guarantee_1}) must be satisfied for every $t = 1, 2, \cdots$. 
\end{enumerate}

